Factored-NeuS: Reconstructing Surfaces, Illumination, and Materials of Possibly Glossy Objects

We develop a method that recovers the surface, materials, and illumination of a scene from its posed multi-view images. In contrast to prior work, it does not require any additional data and can handle glossy objects or bright lighting. It is a progressive inverse rendering approach, which consists of three stages. In the first stage, we reconstruct the scene radiance and signed distance function (SDF) with a novel regularization strategy for specular reflections. We propose to explain a pixel color using both surface and volume rendering jointly, which allows for handling complex view-dependent lighting effects for surface reconstruction. In the second stage, we distill light visibility and indirect illumination from the learned SDF and radiance field using learnable mapping functions. Finally, we design a method for estimating the ratio of incoming direct light reflected in a specular manner and use it to reconstruct the materials and direct illumination. Experimental results demonstrate that the proposed method outperforms the current state-of-the-art in recovering surfaces, materials, and lighting without relying on any additional data.

==> figs/abaltion_fig.tex <==
\newcommand{\ww}{0.15} % 0.14
\newcommand{\iw}{0.8}  % 0.8
\newcommand{\ow}{1.1}  % 1.1
%first line
\begin{minipage}[t]{\ww\linewidth}
% \vspace{3mm}
\subfigure{
    %left title 1
    \rotatebox{90}{\scriptsize{~~~~~~~~~~~Albedo}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/indiSG/their_albedo.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure{
    % left title 2
    \rotatebox{90}{\scriptsize{~~~~~~~~~~~Roughness}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/indiSG/their_rough.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure{
    %left title 1
    \rotatebox{90}{\scriptsize{~~~~~~~~~~~Rendering}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/indiSG/their_rgb.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure[IndiSG]{
    %left title 1
    \rotatebox{90}{\scriptsize{~~~~~Light}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/indiSG/indisg.png}
    \end{minipage}
}
\end{minipage}
\ \ \ 
% \hfill
\vline
% \hfill
\ 
% \vline
\begin{minipage}[t]{\ww\linewidth}
% \vspace{3mm}
\subfigure{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Albedo}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/gt/gt_albedo.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure{
    % left title 2
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Roughness}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/gt/gt_rough.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Rendering}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/gt/gt_rgb.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure[GT]{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~Light}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/gt/sunset.png}
    \end{minipage}
}
\end{minipage}
% \vline
\begin{minipage}[t]{\ww\linewidth}
% \vspace{3mm}
\subfigure{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Albedo}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt-3mlp/our_albedo.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure{
    % left title 2
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Roughness}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt-3mlp/our_rough.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Rendering}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt-3mlp/our_rgb.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure[(1)]{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~Light}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt-3mlp/woSaLvis0or1woW.png}
    \end{minipage}
}
\end{minipage}
% \vline
\begin{minipage}[t]{\ww\linewidth}
% \vspace{3mm}
\subfigure{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Albedo}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt/our_albedo.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure{
    % left title 2
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Roughness}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt/our_rough.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Rendering}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt/our_rgb.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure[(2))]{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~Light}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt/woSaLvis0or1.png}
    \end{minipage}
}
\end{minipage}
% \vline
\begin{minipage}[t]{\ww\linewidth}
% \vspace{3mm}
\subfigure{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Albedo}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our-sa/our_albedo.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure{
    % left title 2
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Roughness}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our-sa/our_rough.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Rendering}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our-sa/our_rgb.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure[(3))]{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~Light}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our-sa/woSa.png}
    \end{minipage}
}
\end{minipage}
% \vline
\begin{minipage}[t]{\ww\linewidth}
% \vspace{3mm}
\subfigure{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Albedo}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our/our_albedo.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure{
    % left title 2
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Roughness}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our/our_rough.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~~~~~~~Rendering}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our/our_rgb.png}
    \end{minipage}
}
% \vspace{-5mm}
\subfigure[(4))]{
    %left title 1
    % \rotatebox{90}{\scriptsize{~~~~~Light}}
    \begin{minipage}[t]{\iw\linewidth}
        \centering
        \includegraphics[width=\ow\linewidth]{exp_figs/ablation/hotdog/our/wSa.png}
    \end{minipage}
}
\end{minipage}


% \begin{minipage}[t]{0.8\linewidth}
% \subfigure{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/gt/gt_albedo.png}
%     \end{minipage}
% }
% \subfigure{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt-3mlp/our_albedo.png}
%     \end{minipage}
% }
% \subfigure{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt/our_albedo.png}
%     \end{minipage}
% }
%     \subfigure{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our-sa/our_albedo.png}
%     \end{minipage}
% }
% \subfigure{
% \begin{minipage}[t]{0.14\linewidth}
%     \centering
%     \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our/our_albedo.png}
% \end{minipage}
% }


% \vspace{-5mm}
% % second line

% \subfigure{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/gt/gt_rough.png}
%     \end{minipage}
% }
% \subfigure{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt-3mlp/our_rough.png}
%     \end{minipage}
% }
% \subfigure{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt/our_rough.png}
%     \end{minipage}
% }
%     \subfigure{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our-sa/our_rough.png}
%     \end{minipage}
% }
%     \subfigure{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our/our_rough.png}
%     \end{minipage}
% }

% %third line
% \vspace{-5mm}

% \subfigure{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/gt/gt_rgb.png}
%     \end{minipage}
% }
% \subfigure{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt-3mlp/our_rgb.png}
%     \end{minipage}
% }
% \subfigure{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt/our_rgb.png}
%     \end{minipage}
% }
% \subfigure{
% \begin{minipage}[t]{0.14\linewidth}
%     \centering
%     \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our-sa/our_rgb.png}
% \end{minipage}
% }
% \subfigure{
% \begin{minipage}[t]{0.14\linewidth}
%     \centering
%     \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our/our_rgb.png}
% \end{minipage}
% }

% \vspace{-5mm}
% \setcounter{subfigure}{0}

% \subfigure[GT]{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/gt/sunset.png}
%     \end{minipage}
% }
% \subfigure[woSa lvis0or1 noWgt]{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt-3mlp/woSaLvis0or1woW.png}
%     \end{minipage}
% }
% \subfigure[woSa lvis0or1]{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our-sa-inteLgt/woSaLvis0or1.png}
%     \end{minipage}
% }
%     \subfigure[woSa]{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our-sa/woSa.png}
%     \end{minipage}
% }
%     \subfigure[Ours]{
%     \begin{minipage}[t]{0.14\linewidth}
%         \centering
%         \includegraphics[width=1.1\linewidth]{exp_figs/ablation/hotdog/our/wSa.png}
%     \end{minipage}
% }
% \end{minipage}

==> figs/ablation_tab_fig.tex <==
\subfigure[ablation tab]{
\begin{minipage}[t]{0.95\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{exp_figs/ablation_tab_fig/ablation.png}
\end{minipage}
}

==> figs/limitation_fig.tex <==
\subfigure[\invrender]{
%left title 1
\rotatebox{90}{\scriptsize{~~~~~~~~Roughness}}
\begin{minipage}[t]{0.14\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/indiSG_vs_ours/hotdog/their_rough.png}
\end{minipage}
}
\subfigure[Ours]{
\begin{minipage}[t]{0.14\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/indiSG_vs_ours/hotdog/our_rough.png}
\end{minipage}
}
\subfigure[GT]{
\begin{minipage}[t]{0.14\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/indiSG_vs_ours/hotdog/gt_rough.png}
\end{minipage}
}
\subfigure[\invrender]{
\begin{minipage}[t]{0.14\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/indiSG_vs_ours/chair/their_rough.png}
\end{minipage}
}
\subfigure[Ours]{
\begin{minipage}[t]{0.14\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/indiSG_vs_ours/chair/our_rough.png}
\end{minipage}
}
\subfigure[GT]{
\begin{minipage}[t]{0.14\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/indiSG_vs_ours/chair/gt_rough.png}
\end{minipage}
}


==> figs/nerfactor_var_fig.tex <==
%first line
\subfigure{
    %left title 1
\rotatebox{90}{\scriptsize{~~~~~~~~~Albedo}}
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/drums/their_albedo.png}
\end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/drums/our_albedo.png}
\end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/drums/gt_albedo.png}
\end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/ficus/their_albedo.png}
\end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/ficus/our_albedo.png}
\end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/ficus/gt_albedo.png}
\end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/lego/their_albedo.png}
\end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/lego/our_albedo.png}
\end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/lego/gt_albedo.png}
\end{minipage}
}
    
\vspace{-3mm}
\setcounter{subfigure}{0}
% second line
\subfigure{
    %left title 1
    \rotatebox{90}{\scriptsize{~~~~~~Rendering}}
    \begin{minipage}[t]{0.09\linewidth}
        \centering
        \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/drums/their_rgb.png}
    \end{minipage}
}
\subfigure{
    \begin{minipage}[t]{0.09\linewidth}
        \centering
        \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/drums/our_rgb.png}
    \end{minipage}
}
\subfigure{
    \begin{minipage}[t]{0.09\linewidth}
        \centering
        \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/drums/gt_rgb.png}
    \end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/ficus/their_rgb.png}
\end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/ficus/our_rgb.png}
\end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/ficus/gt_rgb.png}
\end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/lego/their_rgb.png}
\end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/lego/our_rgb.png}
\end{minipage}
}
\subfigure{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/lego/gt_rgb.png}
\end{minipage}
}
%third line
\setcounter{subfigure}{0}

\subfigure[\invrender]{
%left title 1
\rotatebox{90}{\scriptsize{~~~~~~~~Normal}}
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/drums/their_normal.png}
\end{minipage}
}
\subfigure[Ours]{
    \begin{minipage}[t]{0.09\linewidth}
        \centering
        \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/drums/our_normal.png}
    \end{minipage}
}
\subfigure[GT]{
    \begin{minipage}[t]{0.09\linewidth}
        \centering
        \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/drums/gt_normal.png}
    \end{minipage}
}
\subfigure[\invrender]{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/ficus/their_normal.png}
\end{minipage}
}
\subfigure[Ours]{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/ficus/our_normal.png}
\end{minipage}
}
\subfigure[GT]{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/ficus/gt_normal.png}
\end{minipage}
}
\subfigure[\invrender]{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/lego/their_normal.png}
\end{minipage}
}
\subfigure[Ours]{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/lego/our_normal.png}
\end{minipage}
}
\subfigure[GT]{
\begin{minipage}[t]{0.09\linewidth}
    \centering
    \includegraphics[width=1.2\linewidth]{exp_figs/runOn_nerfactor_data/lego/gt_normal.png}
\end{minipage}
}


==> figs/nerfsyn_var_fig.tex <==
%first line
\subfigure{
    %left title 1
    \rotatebox{90}{\scriptsize{~~~~~~~~~~~~~Albedo}}
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/baloon/their_albedo.png}
    \end{minipage}
}
\subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/baloon/our_albedo.png}
    \end{minipage}
}
\subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/baloon/gt_albedo.png}
    \end{minipage}
}
    \subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/hotdog/their_albedo.png}
    \end{minipage}
}
    \subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/hotdog/our_albedo.png}
    \end{minipage}
}
    \subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/hotdog/gt_albedo.png}
    \end{minipage}
}
%\vspace{-3mm}
\setcounter{subfigure}{0}
% second line
\subfigure{
    % left title 2
    \rotatebox{90}{\scriptsize{~~~~~~~~~~~~~Rendering}}
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/baloon/their_rgb.png}
    \end{minipage}
}
\subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/baloon/our_rgb.png}
    \end{minipage}
}
\subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/baloon/gt_rgb.png}
    \end{minipage}
}
    \subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/hotdog/their_rgb.png}
    \end{minipage}
}
    \subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/hotdog/our_rgb.png}
    \end{minipage}
}
    \subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/hotdog/gt_rgb.png}
    \end{minipage}
}
%third line
\subfigure{
    %left title 1
    \rotatebox{90}{\scriptsize{~~~~~~~~~~~~~Albedo}}
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/chair/their_albedo.png}
    \end{minipage}
}
\subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/chair/our_albedo.png}
    \end{minipage}
}
\subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/chair/gt_albedo.png}
    \end{minipage}
}
    \subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/jug/their_albedo.png}
    \end{minipage}
}
    \subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/jug/our_albedo.png}
    \end{minipage}
}
    \subfigure{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/jug/gt_albedo.png}
    \end{minipage}
}

%\vspace{-3mm}
\setcounter{subfigure}{0}
% fourth line
\subfigure[indiSG]{
    % left title 2
    \rotatebox{90}{\scriptsize{~~~~~~~~~~~~~Rendering}}
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/chair/their_rgb.png}
    \end{minipage}
}
\subfigure[Ours]{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/chair/our_rgb.png}
    \end{minipage}
}
\subfigure[GT]{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/chair/gt_rgb.png}
    \end{minipage}
}
    \subfigure[indiSG]{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/jug/their_rgb.png}
    \end{minipage}
}
    \subfigure[Ours]{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/jug/our_rgb.png}
    \end{minipage}
}
    \subfigure[GT]{
    \begin{minipage}[t]{0.14\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{exp_figs/indiSG_vs_ours/jug/gt_rgb.png}
    \end{minipage}
}

==> figs/sk3d_fig.tex <==
%first line
	\subfigure{
		%left title 1
        \rotatebox{90}{\scriptsize{~~~~~~~~~DTU97}}
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ref_img/97.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ours/97.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/neus/97.png}
		\end{minipage}
	}	
        \subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1.1\linewidth]{exp_figs/neus_vs_ours/geoneus/97.png}
		\end{minipage}
	}	
        \subfigure{
		%left title 1
        \rotatebox{90}{\scriptsize{~~~~~~~~~DTU63}}
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ref_img/63.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1.2\linewidth]{exp_figs/neus_vs_ours/ours/63.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1.2\linewidth]{exp_figs/neus_vs_ours/neus/63.png}
		\end{minipage}
	}	
        \subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1.2\linewidth]{exp_figs/neus_vs_ours/geoneus/63.png}
		\end{minipage}
	}	


        %second line
        \subfigure{
		%left title 1
        \rotatebox{90}{\scriptsize{~~~~~~~~~~DTU110}}
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ref_img/110.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ours/110.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/neus/110.png}
		\end{minipage}
	}	
        \subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1.03\linewidth]{exp_figs/neus_vs_ours/geoneus/110.png}
		\end{minipage}
	}	
        \subfigure{
		%left title 1
        \rotatebox{90}{\scriptsize{~~~~~~~~~~~~~DTU122}}
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ref_img/122.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ours/122.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/neus/122.png}
		\end{minipage}
	}	
        \subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1.05\linewidth]{exp_figs/neus_vs_ours/geoneus/122.png}
		\end{minipage}
	}	
    
    % third line
    \subfigure{
        % left title 2
		\rotatebox{90}{\scriptsize{~~~~~~~~~~~~~funnel}}
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ref_img/funnel.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ours/funnel.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/neus/funnel.png}
		\end{minipage}
	}  
        \subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=0.98\linewidth]{exp_figs/neus_vs_ours/geoneus/funnel.png}
		\end{minipage}
	}  
	\subfigure{
		%left title 1
        \rotatebox{90}{\scriptsize{~~~~~~~~~~~~~pot}}
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ref_img/pot.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ours/pot.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/neus/pot.png}
		\end{minipage}
	}
        \subfigure{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/geoneus/pot.png}
		\end{minipage}
	}

    %\vspace{-4mm}
    \setcounter{subfigure}{0}
    
    \subfigure[Image]{
		%left title 1
        \rotatebox{90}{\scriptsize{~~~~~~snowman}}
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ref_img/snowman.png}
		\end{minipage}
	}
	\subfigure[Ours]{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ours/snowman.png}
		\end{minipage}
	}
	\subfigure[NeuS]{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/neus/snowman.png}
		\end{minipage}
	}
        \subfigure[Geo]{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/geoneus/snowman.png}
		\end{minipage}
	}
        \subfigure[Image]{
		%left title 1
        \rotatebox{90}{\scriptsize{~~~~~~~jug}}
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ref_img/jug.png}
		\end{minipage}
	}
	\subfigure[Ours]{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/ours/jug.png}
		\end{minipage}
	}
	\subfigure[NeuS]{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/neus/jug.png}
		\end{minipage}
	}
        \subfigure[Geo]{
		\begin{minipage}[t]{0.1\linewidth}
			\centering
			\includegraphics[width=1\linewidth]{exp_figs/neus_vs_ours/geoneus/jug.png}
		\end{minipage}
	}

==> tables/ablation.tex <==
% \begin{tabular}{lcccccccccccccccccccccccccc}
% \toprule
% Method & \multicolumn{3}{|c|}{baloons} & \multicolumn{3}{|c|}{hotdog} & \multicolumn{3}{|c|}{chair} & \multicolumn{3}{|c|}{jug} & \multicolumn{3}{|c}{Mean} \\
% \midrule
% & Alb & Rough & Rend & Alb & Rough & Rend & Alb & Rough & Rend & Alb & Rough & Rend & Alb & Rough & Rend\\
% \midrule
% % \multirow{3}*{Fidelity} 
% % 	& 
% OURS--3MLP--integrated light(2)--$S_a$(3) & 23.5666 & 16.8602 & 28.8732   &	29.3118 & 16.9845 &	35.4828	  &	24.8306 & 18.5632 & 32.1460	&	19.6456 & 15.0492 & 33.7829	  &	24.3386 & 16.8642 & 32.5712 \\
% % 	& 
% OURS--integrated light(2)--$S_a$(3) & 23.7817 &16.6445 & 29.1368      &	29.6402 & 17.8643 & 36.3677	      &	24.6260 & 18.7395 & 32.1901	&	19.6636 & 14.7664 & 33.8805    & 24.4278 & 17.0036 & 32.8937 \\
% % 	& 
% OURS--$S_a$(3) & 24.0928 & 23.9876 & 28.8267  &	30.5883 & 18.8354 & 36.0559	      &	25.2399 & 23.1870 & 32.6439	      &	19.6442 & 15.0814 & 33.5659	      &	24.8913 & 20.2728 & 32.7731 \\
% % 	& 
% OURS & 25.7937 & 19.7541 & 33.8933    &	30.0836 & 23.1042 & 36.7112 	& 26.3300 & 15.2441 & 34.5827	  &	22.9494 & 13.0580 & 36.4836 &		26.2891 & 17.7901 & 35.4177\\
% % 	& 
% \bottomrule
% \end{tabular}

\begin{tabular}{lcccccccccccccccccccccccccc}
\toprule
Method & \multicolumn{3}{|c|}{baloons} & \multicolumn{3}{|c|}{hotdog} & \multicolumn{3}{|c|}{chair} & \multicolumn{3}{|c|}{jug} & \multicolumn{3}{|c}{Mean} \\
& Alb & Rough & Rend & Alb & Rough & Rend & Alb & Rough & Rend & Alb & Rough & Rend & Alb & Rough & Rend\\
\midrule
% \multirow{3}*{Fidelity} 
% 	& 
OURS--improved surface--improved vis--$S_a$ & 23.56 & 16.86 & 28.87   &	29.31 & 16.98 &	35.48	  &	24.83 & 18.56 & 32.14	&	19.64 & 15.04 & 33.78	  &	24.33 & 16.86 & 32.57 \\
% 	& 
OURS--improved vis--$S_a$ & 23.78 &16.64 & 29.13      &	29.64 & 17.86 & 36.36	      &	24.62 & 18.73 & 32.19	&	19.66 & 14.76 & 33.88    & 24.42 & 17.00 & 32.89 \\
% 	& 
OURS--$S_a$ & 24.09 & 23.98 & 28.82  &	30.58 & 18.83 & 36.05	      &	25.23 & 23.18 & 32.64	      &	19.64 & 15.08 & 33.56	      &	24.89 & 20.27 & 32.77 \\
% 	& 
OURS & 25.79 & 19.75 & 33.89    &	30.76 & 23.10 & 36.71 	& 26.33 & 15.24 & 34.58	  &	22.94 & 13.05 & 36.48 &		26.28 & 17.79 & 35.41\\
% 	& 
\bottomrule
\end{tabular}

% \begin{tabular}{lcccccccccccccccccccccccccc}
% \toprule
% Method  & \multicolumn{3}{|c|}{OURS--3MLP--integrated light(2)--$S_a$(3)} & \multicolumn{3}{|c|}{OURS--integrated light(2)--$S_a$(3)} & \multicolumn{3}{|c|}{OURS--$S_a$(3)} & \multicolumn{3}{|c}{OURS} \\
% \midrule
%         & Alb & Rough & Rend    & Alb & Rough & Rend      & Alb & Rough & Rend    & Alb & Rough & Rend \\
% \midrule
% ballons  & 23.5666 & 16.8602 & 28.8732       &	29.3118 & 16.9845 &	35.4828	      &	24.8306 & 18.5632 & 32.1460	      &	19.6456 & 15.0492 & 33.7829	      &	24.3386 & 16.8642 & 32.5712 \\
% % 	& 
% hotdog   & 23.7817 &16.6445 & 29.1368        &	29.6402 & 17.8643 & 36.3677	      &	24.6260 & 18.7395 & 32.1901       &	19.6636 & 14.7664 & 33.8805       & 24.4278 & 17.0036 & 32.8937 \\
% % 	& 
% chair    & 24.0928 & 23.9876 & 28.8267       &	30.5883 & 18.8354 & 36.0559	      &	25.2399 & 23.1870 & 32.6439	      &	19.6442 & 15.0814 & 33.5659	      &	24.8913 & 20.2728 & 32.7731 \\
% % 	& 
% jug & 25.7937 & 19.7541 & 33.8933       &	30.0836 & 23.1042 & 36.7112 	  & 26.3300 & 15.2441 & 34.5827	      &	22.9494 & 13.0580 & 36.4836        & 26.2891 & 17.7901 & 35.4177\\
% % 	& 
% mean & 
% \bottomrule
% \end{tabular}


==> tables/ablation_lgt.tex <==
\begin{tabular}{lccccccccc}
    \toprule
            OURS--improved surface--improved vis--$S_a$ & OURS--improved vis--$S_a$ & OURS–$S_a$(3) & OURS \\
    \midrule
           23.4775 & 23.4130 & 23.5048 & 20.2399 \\
    \bottomrule
\end{tabular}

==> tables/ablation_mesh.tex <==
\begin{tabular}{cccc}
\toprule[0.4pt]
NeuS & 1Vol + 1Sur & 1Vol + 2Vol & Ours (full) \\
\midrule[0.2pt]
2.09 & 2.01 & 1.91 & \textbf{1.88} \\
\bottomrule[0.5pt]
\end{tabular}

==> tables/capabilities.tex <==
\begin{tabular}{lcccccccccccccccc}
\toprule
Method & \makecell{Explicit surface \\ extraction} & \makecell{Diffuse/specular \\ color decomposition} & \makecell{Illumination \\ reconstruction} & \makecell{Materials \\ reconstruction} & \makecell{Handles glossy \\ surfaces} & No Extra Data? & \makecell{Code \\ available} & Venue \\
\midrule
% RefNeRF~\cite{Refnerf} & \XSolidBrush & \Checkmark \\
NeRV~\cite{Nerv} & \XSolidBrush & \Checkmark & \Checkmark & \Checkmark & \XSolidBrush & \Checkmark & [\href{https://pratulsrinivasan.github.io/nerv/}{to appear}] & CVPR 2021 \\
PhySG~\cite{Physg} & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & object masks & \href{https://github.com/Kai-46/PhySG}{\Checkmark} & CVPR 2021 \\
NeuS~\cite{NeuS} & \Checkmark & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \Checkmark & \href{https://github.com/Totoro97/NeuS}{\Checkmark} & NeurIPS 2021 \\
NeRFactor~\cite{Nerfactor} & \XSolidBrush & \Checkmark & \Checkmark & \Checkmark & \XSolidBrush & BRDF dataset  & \href{https://github.com/google/nerfactor}{\Checkmark} & SG Asia 2021 \\
Ref-NeRF~\cite{Refnerf} & \XSolidBrush & \Checkmark & \XSolidBrush & \XSolidBrush & \Checkmark & \Checkmark & \href{https://github.com/google-research/multinerf}{\Checkmark} & CVPR 2022 \\
NVDiffrec~\cite{NVDiffrec} & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \XSolidBrush & object masks & \href{https://github.com/NVlabs/nvdiffrec}{\Checkmark} & CVPR 2022 \\
IndiSG~\cite{Indirect} & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \XSolidBrush & object masks & \href{https://github.com/zju3dv/invrender}{\Checkmark} & CVPR 2022 \\
% NeILF & \XSolidBrush &  &  &  &  & Normals, & \href{https://github.com/apple/ml-neilf}{\Checkmark} & ECCV 2022 \\
Geo-NeuS~\cite{geo-neus} & \Checkmark & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & point clouds & \href{https://github.com/GhiXu/Geo-Neus}{\Checkmark} & NeurIPS 2022 \\
% \midrule
BakedSDF~\cite{Bakedsdf} & \Checkmark & \Checkmark & \XSolidBrush & \XSolidBrush & \XSolidBrush & \Checkmark & \XSolidBrush & SG 2023 \\
TensoIR~\cite{TensoIR} & \XSolidBrush & \Checkmark & \Checkmark & \Checkmark & \XSolidBrush & \Checkmark & \href{https://github.com/Haian-Jin/TensoIR}{\Checkmark} & CVPR 2023 \\
NeFII~\cite{Nefii} & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \XSolidBrush & \Checkmark & \XSolidBrush & CVPR 2023 \\
% NDJIR~\cite{Ndjir} & \Checkmark & \Checkmark & \Checkmark & \XSolidBrush & \XSolidBrush & \Checkmark & TODO & arXiv 2023/02 \\ % Has considerably worse Chamfer distance than NeuS on DTU
Ref-NeuS~\cite{Refneus} & \Checkmark & \XSolidBrush & \XSolidBrush & \XSolidBrush & \Checkmark & \Checkmark & [\href{https://g3956.github.io/}{to appear}] & arXiv 2023/03 \\
% VDN-NeRF~\cite{VDN-NeRF} & \Checkmark & \XSolidBrush & \XSolidBrush & \XSolidBrush & \Checkmark & \Checkmark & \href{https://github.com/BoifZ/VDN-NeRF}{\Checkmark} & arXiv 2023/03 \\
$\alpha$Surf~\cite{AlphaSurf} & \Checkmark & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & object masks & [\href{https://alphasurf.netlify.app/}{to appear}] & arXiv 2023/03 \\
NeILF++~\cite{NeILF++} & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \XSolidBrush & \Checkmark & [\href{https://yoyo000.github.io/NeILF_pp/}{to appear}] & arXiv 2023/03 \\
ENVIDR~\cite{Envidr} & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & BRDF dataset & [\href{https://github.com/nexuslrf/ENVIDR}{to appear}] & arXiv 2023/03 \\
NeMF~\cite{NeMF} & \XSolidBrush & \Checkmark & \Checkmark & \Checkmark & \XSolidBrush & \Checkmark & \XSolidBrush & arXiv 2023/04 \\
NeAI~\cite{NeAI} & \XSolidBrush & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & [\href{https://yiyuzhuang.github.io/NeAI/}{to appear}] & arXiv 2023/04 \\
NeRO~\cite{nero} & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & arXiv 2023/05 \\
% \midrule
\modelname (ours) & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & [in supp] & - \\
\bottomrule
\end{tabular}


==> tables/chamfer_distance_dtu.tex <==
\begin{tabular}{cccccc}
    \toprule
           & dtu63 & dtu97 &dtu110 &dtu122  & Mean\\
    \midrule
    % IDR  & x & x & x  & x & x & x & x & x\\
    NeuS  & 1.01 & 1.21 & 1.14  & 0.54 & 0.98 \\
    Geo-NeuS  & 0.96 & 0.91 & 0.70  & 0.37 & 0.73 \\
    \midrule
    IndiSG  & 1.15 & 2.07 & 2.60 & 0.61  & 1.61\\
    OURS   & 0.99  & 1.15 & 0.89 & 0.46 & 0.87 \\
    \bottomrule
\end{tabular}

==> tables/chamfer_distance_sk3d.tex <==
\begin{tabular}{cccccc}
    \toprule
       ($10^{-3}$)    &  pot & funnel & snowman &jug & Mean\\
    \midrule
    % IDR  & x & x & x  & x & x & x & x & x\\
    NeuS   & 2.09 & 3.93 & 1.40 & 1.81  & 2.31\\
    Geo-NeuS   & 1.88 & 2.03 & 1.64 & 1.68  & 1.81\\
    \midrule
    IndiSG  & x & x & x & x  & x\\
    % Ref-NeRF    & x & x & x  & x  & x\\
    OURS   & 1.54 & 1.95 & 1.31 & 1.40  & 1.55\\
    \bottomrule
\end{tabular}

==> tables/dtu.tex <==
\begin{tabular}{lcccccccccccccccc}
\toprule
% 	Metric & 
% \multirow{2}{*}{Method} & \multicolumn{15}{c}{Scene ID} \\
% & 24 & 37 & 40 & 55 & 63 & 65 & 69 & 83 & 97 & 105 & 106 & 110 & 114 & 118 & 122 & \textbf{Mean} \\
Method & 24 & 37 & 40 & 55 & \todo{63} & 65 & 69 & 83 & \todo{97} & 105 & 106 & \todo{110} & 114 & 118 & \todo{122} & \textbf{Mean} \\
\midrule
% 	\multirow{4}*{Fidelity} 
NeRF   & 1.90 & 1.60 & 1.85 & 0.58 & 2.28 & 1.27 & 1.47 & 1.67 & 2.05 & 1.07 & 0.88 & 2.53 & 1.06 & 1.15 & 0.96 & 1.49 \\
% 	& 
VOLSDF & 1.14 & 1.26 & 0.81 & 0.49 & 1.25 & 0.70 & 0.72 & 1.29 & 1.18 & 0.70 & 0.66 & 1.08 & 0.42 & 0.61 & 0.55 & 0.86 \\
% 	& 
NeuS   & 1.00 & 1.37 & 0.93 & 0.43 & 1.10 & 0.65 & \textbf{0.57} & 1.48 & 1.09 & 0.83 & 0.52 & 1.20 & 0.35 & \textbf{0.49} & 0.54 & 0.84 \\
% 	& 
HF-NeuS   & 0.76 & 1.32 & 0.70 & 0.39 & 1.06 & \textbf{0.63} & 0.63 & \textbf{1.15} & 1.12 & 0.80 & 0.52 & 1.22 & \textbf{0.33} & \textbf{0.49} & 0.50 & 0.77 \\
% 	& OURS   & \textbf{0.63} & \textbf{1.04} & 0.96 & 0.42 & \textbf{1.00} & 0.87 & 0.75 & 1.38 & 1.19 & 0.81 & 0.57 & 1.38 & 0.41 & 0.54 & 0.55 & 0.83 \\
% 	& 
\modelname\ (ours)   & - & - & - & - & 0.99 & - & - & - & 1.15 & - & - & 0.89 & - & - & 0.46 & - \\
% \modelname\ (ours)   & 0.83 & 1.56 & 0.72 & 0.39 & 0.99 & 0.71 & - & 1.47 & 1.15 & 0.81 & 0.58 & 0.89 & 0.35 & 0.46 & 0.46 & - \\
\midrule
% 	\multirow{4}*{PSNR} 
NeRF   & 26.24 & 25.74 & 26.79 & 27.57 & 31.96 & 31.50 & 29.58 & 32.78 & 28.35 & 32.08 & 33.49 & 31.54 & 31.0 & 35.59 & 35.51 & 30.65 \\
% 	& 
VOLSDF & 26.28 & 25.61 & 26.55 & 26.76 & 31.57 & 31.50 & 29.38 & 33.23 & 28.03 & 32.13 & 33.16 & 31.49 & 30.33 & 34.90 & 34.75 & 30.38 \\
% 	& 
NeuS   & 28.20 & 27.10 & 28.13 & 28.80 & 32.05 & 33.75 & 30.96 & 34.47 & 29.57 & 32.98 & 35.07 & 32.74 & 31.69 & 36.97 &  37.07 & 31.97 \\
% 	& 
HF-NeuS   & 29.15 & 27.33 & 28.37 & 28.88 & 32.89 & \textbf{33.84} & \textbf{31.17} & 34.83 & \textbf{30.06}
& 33.37 & 35.44 & 33.09 & 32.12 & 37.13 & 37.32 & 32.33 \\
%  & 
\modelname\ (ours)   & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
\bottomrule
\end{tabular}

==> tables/nerfactor.tex <==
\begin{tabular}{cccccccccc}
    \toprule
           & \multicolumn{3}{|c|}{drums} & \multicolumn{3}{|c|}{ficus} & \multicolumn{3}{|c}{lego} \\
    \midrule
           & albedo & rendering & normal & albedo & rendering &normal & albedo & rendering & normal \\
    \midrule
    indiSG  & 13.6096 & 18.7547 & 15.3302 & 9.2636 & 23.2154 & 14.2748 & 14.8967 & 26.6837 & 18.3698  \\
    Ours   & 17.7160 & 21.7203 & 16.6569 & 11.2701 & 26.6797 & 14.6935 & 15.6762 & 29.9495 & 19.3429 \\
    \bottomrule
\end{tabular}

==> tables/sk3d.tex <==
\begin{tabular}{lcccccccccccccccc}
	\toprule
% 	Metric & 
	% \multirow{2}{*}{Method} & \multicolumn{15}{c}{Scene ID} \\
 % & 24 & 37 & 40 & 55 & 63 & 65 & 69 & 83 & 97 & 105 & 106 & 110 & 114 & 118 & 122 & \textbf{Mean} \\
	Method & No. & No. & No. & No. & No. & No. & No. & No. & No. & No. & No. & No. & No. & No. & No. & \textbf{Mean} \\
	\midrule
% 	\multirow{4}*{Fidelity} 
% 	& 
	NeuS   & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% 	& 
	HF-NeuS or IDR   & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% 	& OURS   & \textbf{0.63} & \textbf{1.04} & 0.96 & 0.42 & \textbf{1.00} & 0.87 & 0.75 & 1.38 & 1.19 & 0.81 & 0.57 & 1.38 & 0.41 & 0.54 & 0.55 & 0.83 \\
% 	& 
	\modelname\ (ours)   & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
	\midrule
% 	\multirow{4}*{PSNR} 
% 	& 
	NeuS   & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% 	& 
	HF-NeuS or IDR   & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%  & 
 \modelname\ (ours)   & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
	\bottomrule
\end{tabular}
